Erd\"{o}s-Szekeres Partitioning Problem

In this note, we present a substantial improvement on the computational complexity of the Erd\"{o}s-Szekeres partitioning problem and review recent works on dynamic \textsf{LIS}.

==> tables/results.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}

\begin{table}[!htbp]
	\centering
	\begin{tabular}{|l|c|c|}
		\hline
		Problem & Approximation factor & Update time\\
		\hline
		\textsf{LIS} & $1+\epsilon$ & $\tilde O(\sqrt{n})$\\
		\hline	
        \textsf{LIS} & $O((1/\epsilon)^{O(1/\epsilon)})$ & $\tilde O(n^{\epsilon})$\\
	    \hline
	    $\mathsf{LIS}^+$ & $O(\log n)$ & $O(\log^3 n)$\\
	    \hline
		\textsf{DTM} & $1+\epsilon$ & $O(\log^2 n)$\\
        \hline
	\end{tabular}
\caption{The results of this paper are summarized in this table. $\mathsf{LIS}^+$ is a special case of \textsf{LIS} where only element addition is allowed.}
\end{table}



==> tables/runtimes.tex <==
\begin{table}[!htbp]
\centering
\begin{tabular}{|c|c|c|}
	\hline
	Dynamic & worst-case  & approximation \\
	algorithm &  update time &  factor\\
	\hline 
	$\mathcal{A'}_0$ & $\tilde O(n)$ & 1\\
	\hline 
	$\mathcal{A'}_1$ & $\tilde O(n^{2/3+\kappa})$ & $O(1/\kappa)$\\
	\hline
	$\mathcal{A'}_2$ & $\tilde O(n^{1/2+\kappa})$ & $O(1/\kappa^2)$\\
	\hline
	$\mathcal{A'}_3$ & $\tilde O(n^{2/5+\kappa})$ & $O(1/\kappa^3)$\\
	\hline
	\vdots  & \vdots & \vdots \\
	\hline
	$\mathcal{A'}_k$ & $\tilde O(n^{\frac{2}{k+2}+\kappa})$ & $O(1/\kappa^k)$\\
	\hline
\end{tabular}
\caption{Guarantees of the dynamic solutions are shown in this figure.}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
	\hline
	block-based & $m$ & $f(n)$ & $g(n)$ & $h(n)$ & approximation \\
	 algorithm &  & &  &  & factor \\
%	\hline 
%	- & - & -  &- & - & -\\
	\hline
	$\mathcal{A}_1$ & $n^{1/3}$ & $\tilde O(n^{1+\kappa})$ & $n^{2/3}$ & $\tilde O(n^{2/3+\kappa})$ & $O(1/\kappa)$\\
	\hline
	$\mathcal{A}_2$ & $n^{1/4}$ & $\tilde O(n^{1+\kappa})$ & $n^{3/4}$ & $\tilde O(n^{1/2+\kappa})$ & $O(1/\kappa^2)$\\
	\hline
	$\mathcal{A}_3$ & $n^{1/5}$ & $\tilde O(n^{1+\kappa})$ & $n^{4/5}$ & $\tilde O(n^{4/5+\kappa})$ & $O(1/\kappa^3)$\\
	\hline
	\vdots  & \vdots & \vdots & \vdots & \vdots & \vdots \\
	\hline
	$\mathcal{A}_k$ & $n^{\frac{1}{k+2}}$ &$\tilde O(n^{1+\kappa})$ & $n^{\frac{k+1}{k+2}}$ & $\tilde O(n^{\frac{2}{k+2}+\kappa})$ & $O(1/\kappa^k)$\\
	\hline
\end{tabular}
\caption{Guarantees of the block-based solutions are shown in this figure. We assume that the length of the initial array $a$ for the block-based algorithm is $n$.}
\end{table}


